Fault Injection and Safe-Error Attack for Extraction of Embedded Neural Network Models

Model extraction emerges as a critical security threat with attack vectors exploiting both algorithmic and implementation-based approaches. The main goal of an attacker is to steal as much information as possible about a protected victim model, so that he can mimic it with a substitute model, even with a limited access to similar training data. Recently, physical attacks such as fault injection have shown worrying efficiency against the integrity and confidentiality of embedded models. We focus on embedded deep neural network models on 32-bit microcontrollers, a widespread family of hardware platforms in IoT, and the use of a standard fault injection strategy - Safe Error Attack (SEA) - to perform a model extraction attack with an adversary having a limited access to training data. Since the attack strongly depends on the input queries, we propose a black-box approach to craft a successful attack set. For a classical convolutional neural network, we successfully recover at least 90% of the most significant bits with about 1500 crafted inputs. These information enable to efficiently train a substitute model, with only 8% of the training dataset, that reaches high fidelity and near identical accuracy level than the victim model.

==> source/scope_contribution.tex <==
%\noindent\textbf{Scope and contribution. }
Our scope is the use of fault injection for the purpose of extracting ML models embedded in constrained devices. Typically, we consider 32-bit microcontroller (ARM Cortex-M) platforms. For such platforms based on Flash memory, bit-flips with rowhammer as in~\cite{deepsteal2022} are not practicable. However, our work is the first to demonstrate that a different attack strategy is possible and can reach consistent results regarding the state-of-the-art. Our contributions are the following:

\begin{itemize}[nosep]
    \item We demonstrate a new extraction method based on a Safe-Error Attack (SEA) that exploits a bit-set fault model ($\texttt{0}\rightarrow\texttt{1}$, $\texttt{1}\rightarrow\texttt{1}$). SEA enables to recover the most significant bit values of the victim model parameters. These information enable to efficiently constrain the substitute model training, even with limited data.
    \item We use full 8-bit quantized models %(parameters, activation functions and scores) 
    as for real-world embedded applications, a setting that makes our approach more challenging.
    \item We show that the model inputs significantly impact extraction performance and we propose an input generation method to increase the recovery rate. 
\end{itemize}
\text{ }

\noindent\textbf{Availability.} Data and codes related to our work are publicly available on \url{https://anonymous.4open.science/r/SEA\_for\_Extraction\_of\_DNNs-1048}.


 

==> tab/model_architecture.tex <==
\begin{table}[h!]
\centering
\caption{MLP (MNIST) and CNN (Cifar-10) architecture. We follow the PyTorch naming for fully-connected layers with "Linear". Convolutional layers are composed by 5x5 kernels and followed by a pooling layer (average 2x2).}
\label{model_architecture}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccc}
\toprule
Layer & \# param & Layer & \# param  \\
\midrule
Inputs (784)& & Inputs (32,32) & \\
Linear 1 (128 neurons), ReLU & 100352 & Conv1 (32 kernels), ReLU & 2400  \\
Linear 2 (64 neurons), ReLU & 8192 & Conv2 (32 kernels), ReLU & 25600  \\
Linear 3 (10 neurons), Softmax & 640 & Conv3 (64 kernels), ReLU & 51200  \\
 & &   Linear (10 neurons), Softmax & 10240  \\
\midrule
MLP & 109184 & CNN & 89440\\
\bottomrule
\end{tabular}
%}
\end{table}


==> tab/tab_prediction_cifar10.tex <==
\begin{table}[b]
\caption{Bit-recovery efficiency for \textit{No-doubt} and \textit{Ambiguous} test inputs. CNN model (Cifar-10) over 3000 inputs}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Layers} & \multicolumn{2}{c}{No recovery (\%)} & \multicolumn{2}{c}{\# of bits recovered} \\
& No-doubt & Ambiguous & No-doubt & Ambiguous \\
\midrule
Conv. 1 & 14.03 & 0.0 & 383 (888) & 7176 (1315) \\
Conv. 2 & 68.2 & 0.0 & 835 (4129) & 32902 (11819) \\
Conv. 3 & 79.03 & 0.0 & 341 (2139) & 15260 (9690) \\
Linear 1 & 66.7 & 0.0 & 23 (92) & 804 (410) \\
\midrule
Model  & 13.93 & 0.0 & 1583 (7003) & 56142 (21595) \\
\bottomrule
\end{tabular}
}
\label{tab_prediction_cifar10}
\end{center}
\end{table}

==> tab/tab_prediction_mnist.tex <==
\begin{table}[b]
\caption{Bit-recovery efficiency for \textit{No-doubt} and \textit{Ambiguous} test inputs. MLP model (MNIST) over \textcolor{red}{500 ?} inputs}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Layers} & \multicolumn{2}{c}{No recovery (\%)} & \multicolumn{2}{c}{\# of bits recovered} \\
& No-doubt & Ambiguous & No-doubt & Ambiguous \\
\midrule
Linear 1 & 99.0 & 0.0 & 12 (229) & 10530 (7356) \\
Linear 2 & 98.6 & 0.0 & 2 (37) & 2879 (1490) \\
Linear 3 & 78.4 & 0.0 & 3 (10) & 290 (93) \\
\midrule
Model  & 78.4 & 0.0 & 17 (273) & 13699 (7356) \\
\bottomrule
\end{tabular}
}
\label{tab_prediction_mnist}
\end{center}
\end{table}

==> tab/tab_prediction_mnist_cifar10.tex <==
\begin{table}[b!]
\caption{Bit-recovery efficiency for \textit{Certain} and \textit{Uncertain} test inputs.}
\begin{center}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{lll|rr}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{l}{No recovery (\%)} & \multicolumn{2}{r}{Average \# of bits recovered (std)} \\
& Certain & Uncertain & Certain & Uncertain \\
\midrule
MLP  & 78.4 & 0.0 & 17 (273) & 13699 (7356) \\
\midrule
CNN  & 13.93 & 0.0 & 1583 (7003) & 56142 (21595) \\
\bottomrule
\end{tabular}
%}
\label{tab_prediction_mnist_cifar10}
\end{center}
\end{table}
